When to Read Documents or QA History: On Unified and Selective Open-domain QA

This paper studies the problem of open-domain question answering, with the aim of answering a diverse range of questions leveraging knowledge resources. Two types of sources, QA-pair and document corpora, have been actively leveraged with the following complementary strength. The former is highly precise when the paraphrase of given question $q$ was seen and answered during training, often posed as a retrieval problem, while the latter generalizes better for unseen questions. A natural follow-up is thus leveraging both models, while a naive pipelining or integration approaches have failed to bring additional gains over either model alone. Our distinction is interpreting the problem as calibration, which estimates the confidence of predicted answers as an indicator to decide when to use a document or QA-pair corpus. The effectiveness of our method was validated on widely adopted benchmarks such as Natural Questions and TriviaQA.

==> 3_model-alt.tex <==
\section{Proposed Method}
In this section, we formally describe DR- and QR-QA as preliminaries (Section 3.1) 
%and  our open-book QA model on QA-pairs (Section 3.2), and propose our unified approach to calibrate and answer over two knowledge sources (Section 3.3 and 3.4).  
and our unification baseline (Section 3.2), followed by our proposed calibration for selective QA (Section 3.3).
% We denote a question as $q$, and answer as $a$.
% As Open-book QA setting, 


\subsection{DR-QA: A Baseline using Documents as Knowledge}

Open-book QA requires to answer question $q$ given context $\mathbf{c}$, \ie, optimizing $\text{P}_{LM}(\mathbf{a}|\mathbf{q}, \mathbf{c})$.
DR-QA~\cite{lee2019latent,karpukhin2020dense} typically uses Wikipedia documents as knowledge $\mathbf{c}$.
In practice, 
% since it is infeasible to insert all corpus into QA models,
\citet{karpukhin2020dense} leverage dense retrieval to retrieve top-$n$ passages $\mathbf{d}_{1:n}$ corresponding to $\mathbf{q}$ and use them as context.
That is, the goal of DR-QA is to find optimal $\text{P}_{LM}(\mathbf{a}|\mathbf{q}, \mathbf{d}_{1:n})$.
% where $\mathbf{d}_{1:n}$ is top-$n$ passages retrieved by the dense retrieval.
% In this paper, we use a generative model to predict answer $a$.

In this paper, as the backbone of DR-QA, we use a state-of-the-art generative reader: Fusion-in-Decoder \cite{izacard2021leveraging}, based on a pretrained language model -- T5~\cite{raffel2020exploring}.
This approach separately encodes top-$n$ passages in an encoder, and fuses them in a decoder.
The final answer $\text{A}$ is obtained as follows:
\begin{equation}
    \begin{split}
    \text{Fuse}(\mathbf{q}, \mathbf{d}_{1:n}) = & ~ [\text{Enc}(\mathbf{q}, \mathbf{d}_{1});,...,;\text{Enc}(\mathbf{q}, \mathbf{d}_{n})] \\
    \text{A} = & ~ \text{Dec (\text{Fuse}}(\mathbf{q}, \mathbf{d}_{1:n}))
    \end{split}
\end{equation}
% \vspace{-2mm}
where Enc and Dec indicate Encoder and Decoder modules in transformer \cite{vaswani2017attention}, and $[~; ]$ indicates the concatenation of encoder's outputs.
Let $\mathbf{x}$ denote the input sequence, and $\mathbf{y} = (y_1,...,y_T)$ the output sequence.
The language model based QA model is trained with maximum likelihood estimation (MLE) to optimize the following objective for a given ($\mathbf{x}$, $\mathbf{y}$): 
\begin{equation}
    \begin{split}
    \mathcal{L}(\mathbf{x},\mathbf{y}) = - \sum_{t=1}^{T} \text{log}~\text{P}_{LM}( y_t |\mathbf{y}_{<t}, \mathbf{x})
    \end{split}
    \label{lm_loss}
\end{equation}
where $\mathbf{x}$ is a pair of question/document $(\mathbf{q},\mathbf{d}_{1:n})$, and $\mathbf{y}$ is the ground-truth answer $\mathbf{a}^*$ in our setting.
Meanwhile, at inference time, we use Greedy Decoding,\footnote{As a decoding method, we can choose beam search or temperature-based sampling, but greedy decoding empirically outperformed others in our QA tasks.} which is commonly used for QA tasks.
A decoded sequence is $\mathbf{\hat{a}}=(\hat{a}_1,\hat{a}_2,...,\hat{a}_T)$, where each token is selected as follows:
\begin{equation}
    \begin{split}
    \hat{a}_t = \argmax_{y \in V} ~ \text{P}_{LM}(y|\mathbf{\hat{a}}_{<t}, \mathbf{q}, \mathbf{d}_{1:n})
    \end{split}
    \label{eq3}
\end{equation}







% source knowledge as $\mathcal{K}_s$, and target as $\mathcal{K}_t$.
% We first build an initial model $\theta^{old}$ pre-trained on source knowledge $\mathcal{K}_s$. 
% Then, we inject target knowledge $\mathcal{K}_t$ into the pre-trained model and obtain the infused model $\theta^{new}$.



% In CBQA, LMs answer factual questions with the implicit knowledge stored in the model, without any external context (\ie, in contrast to open-domain QA), so that LMs are required to adequately update their parameters to the target knowledge.
% In our \task, LMs learn source (original) knowledge first, then update them with target (new) knowledge without source knowledge access.
% For the above setting, source knowledge (to be retained) and target knowledge (to be added) in CuQA do not have any overlap of QA pairs (or paraphrases) for any given fact.




\subsection{Preliminary Experiment: Potential of using QA History as Knowledge}

% Instead of using documents as knowledge, there are several alternative approaches.
Suppose that a user ask any questions in training examples that are already answered, or its paraphrases.
To answer such question, retrieving and reading documents may be inefficient, while matching with a QA-pair in training set is easier and more efficient.
For matching with training examples, 
\citet{roberts2020much} focus on memorization ability of large LMs by proposing a \textit{closed-book QA} task to directly answer questions without any context knowledge, but it requires extremely large models for memorization of all knowledge.
As another approach, \textit{in-context learning} \cite{brown2020language} can improve closed-book QA, by providing few-shot examples in the same task.
% while a recent work~\cite{liu2021makes} shows that task performances depend heavily on the choice of in-context examples.
For a careful choice of in-context examples,
% For a careful choice, 
\citet{liu2021makes} retrieve examples that are semantically similar to a target input, which boosts in-context learning.


Inspired by these trends, we propose an alternative QA task leveraging existing QA corpus and QA-Retrieval without documents.
As shown in Figure \ref{figure1}, we retrieve top-$n$ QA pairs from QA corpus as in-context examples, 
and finetune a QA model with the in-context examples.
Specifically, as QA corpus and QA-Retrieval, we used Probably Asked Questions (PAQ) and a dense retrieval of RePAQ (See Appendix \ref{appendix_retrieval} for more details), which are proposed in \citet{lewis2021paq}.
% \paragraph{QR-QA} leverages a collection of QA pairs as knowledge $\mathbf{c}$.
% As our retrieval for QA-pairs, we used RePAQ \cite{lewis2021paq} based on dense retrieval models on the QA corpus.
% Given a question, the dense retrieval first extracts top-$n$ QA pairs from the corpus, and then selects top-1 QA pair as the final answer corresponding to a given question.
% Instead, we unify Question Retrieval as a DR-QA problem (denoted as \textbf{QR-QA}).
Given a target question, we extract top-$n$ QA-pairs from PAQ and 
the top-$n$ retrieved QA-pairs are provided as context, as if it is a passage retrieved from DR-QA (denoted as $\mathbf{k}$) as below:
\begin{addmargin}[0.6em]{0em}
{\small \texttt{\noindent Question: \kyungjae{\{target $q$\}}, ~ Answer: ~~~~~~~~~~~~ $\backslash$n \\  Question: \kyungjae{\{example $q_1$\}}, Answer: \kyungjae{\{example $a_1$\}} $\backslash$n \\  Question: \kyungjae{\{example $q_2$\}}, Answer: \kyungjae{\{example $a_2$\}} $\backslash$n \\ Question: ~~~ ... ~~~~~ Answer: ~~~ ...}}
\end{addmargin}
% \vspace{2mm}


\begin{figure}[t]
	\centering
	\includegraphics[width=74mm]{figures/figure_preliminary.pdf}
	\caption{Preliminary study on Natural Questions and TriviaQA.}
	\label{figure_preliminary}
\end{figure}

% To unify the two backbones, a naive baseline is pipelining the top-1 answer from one model to another, which performs worse than a single model.
%Instead of such selection, we leverage the top-$n$ QA pairs as additional knowledge, which will be described in the next section.
%In our work, we consider the retrieved top-$n$ QA pairs as additional context for Open-book QA.
%We 

In Figure \ref{figure_preliminary}, we conduct a preliminary experiment to verify the above hypothesis (see Appendix \ref{} for more details on the implementation).
Based on T5-large model, we observe the accuracy (exact match) of the following variants: 
(1) ``Pretrained (zero-shot)'' is closed-book setting and the performances of T5 have shown poor on both benchmarks, which is in contrast to GPT's capability \cite{brown2020language}. 
Meanwhile, (2) ``Pretrained (few-shot)'', adding the few examples retrieved from QA-pair corpus, significantly improves QA performances, and furthermore (3) ``Finetuned (few-shot)'' also boosts the performances.
Finally, to verify the complemantarity with \textbf{DR-QA}, we calculate the upper bound (Union of DR-QA and QR-QA) -- whether both predictions from DR- and QR-QA include a correct answer, or not.
The upper bounds show the potential complemantarity of document and QA-pair corpus, which motivates leveraging both knowledge sources.

% That is, we optimize $\text{P}_{LM}(\mathbf{a}|\mathbf{q}, \mathbf{k})$ in our redefined task.
% This approach has several advantages.
% (1) Leveraging $n$ QA pairs as context enables us to infer the answer more robustly than RePAQ, in that the error of the retrieval result (top-1 QA pair) does not necessarily lead to the failure of question answering.
% (2) A single generative model can be trained on both document and QA pair knowledge, by multi-task learning.


% Additionally, this unified formulation has the advantage in that we can leverage the LM's confidence scores, in the same way as with documents.
% For the decoding function  $\mathcal{F}$ of LM, question $q$ and the retrieved QA pair set $\mathbf{k}$, we formulate our answer as $\mathcal{F}(q, \mathbf{k})$.

% Meanwhile, in QA system that purely relies on QA pair retrieval, the answer is explicitly parsed from the top-1 QA pair \cite{lewis2021paq}.
% In that case, $\mathcal{F}$ in our formulation is replaced with the parsing function, and $\mathbf{k}$ with the top-1 QA pair.

%In this paper, we focus on \textit{Open-book QA} leveraging both document and QA-pair corpus as contexts for a unified generative reader. 
%As shown in Figure \ref{figure1}, we redefine the QA-pair Retrieval task as \textit{Open-book QA}.
%Instead of selecting top1 QA pair as a final answer directly,
%we concatenate the few retrieved QA examples and provide them to QA reader as context.
%This approach has several advantages. 
%It is capable of compensating for retrieval errors. 
%Also, the context of QA pairs could be strong hints in that answer candidates can be presented explicitly if the retrieval succeeds, while answers in documents are implicit with noisy information.


Now that we have two sources $ \mathbf{d}_{1:n}$ and $\mathbf{k}$ as context, our baseline to combine the two is from \cite{oguz2020unik}, which concatenates all knowledge -- texts, tables, and knowledge graphs in the decoder.
Through this ``concat'' baseline, 
we can consider $\mathbf{k}$ of QA-pairs as (\text{n+1})th passage in DR-QA, so that the final answer $A_{base}$ is obtained as follows:
\begin{equation}
    \begin{aligned}
    % \text{Fuse}(\mathbf{q}, \mathbf{d}_{1:n}, \mathbf{k}) = ~  \\
    & A_{base}(\mathbf{q}, \mathbf{d}_{1:n}, \mathbf{k}) = \\ 
    & ~~~~ \text{Dec}([\text{Enc}(\mathbf{q},\mathbf{d}_1);...;\text{Enc}(\mathbf{q},\mathbf{d}_n); \text{Enc}(\mathbf{q},\mathbf{k})])
    % \text{Dec}(\text{Enc}(\mathbf{q}, [\mathbf{d}_{1};...;\mathbf{d}_{n}; \mathbf{k}]))
    \end{aligned}
\end{equation}
where $[~; ]$ indicates the concatenation of encoder's outputs.
However, due to unreliable inputs from the concatenation, the performance may degrade with increasing noise, as reported in~\citet{oguz2020unik}. 
We hypothesize this as a cause of combining multiple knowledge underperforming a single model and propose selective QA.




% Additionally, in our experiment (Sec 4.x), we observed the performance degradation occurs when answer candidates in retrieved QA-pairs act as distractor.
% That is, this naive solution is prone to the shortcut behavior which favors the explicit information in QA-pairs.




% \vspace{-3mm}
% \begin{equation}
%  A_{backoff} = \begin{cases}
%   \mathcal{F}(q, \mathbf{k}) & \text{if~} P_{\mathcal{F}}(a|q,\mathbf{k}) \geq \delta \\
%   \mathcal{G}(q, \mathbf{d}) & \text{otherwise}
%   \end{cases}
%   \label{eq2}
% \end{equation}
% where $P_{\mathcal{F}}(a|q,\mathbf{k})$ is the confidence score of model $\mathcal{F}$, and threshold $\delta$ is a hyper-parameter. Specifically, we denote the retrieved document set as $\mathbf{d}$, and QA-pair set as $\mathbf{k}$.

% However, they have limitation in utilizing the complementarity among the knowledge sources.
% First of all, method (1) does not guarantee that the QA model benefits from the additional knowledge source.
% For example, \citet{oguz2020unik} reports that method (1) often degrades the QA performance in NaturalQuestions and TriviaQA when knowledge graph triplets are added to other knowledge sources.
% In our experiment in [4.x], we show that this degradation is particularly severe when QA pairs are added to documents, and the QA model trained with method (1) is prone to the shortcut behavior which favors the information in QA pairs.
% Meanwhile, method (2) only evaluates reliability of the answer from the single knowledge source, which results in explicitly prioritizing one knowledge source over others.
% The drawback of back-off based model is that the performance depends on the manual choice of the threshold $\delta$, and other knowledge sources are ignored without evaluation if $P_{\mathcal{F}}(a|q,\mathbf{k})$ is above $\delta$. \cite{lewis2021paq}

\subsection{Selective QA via Calibration}

%We diagnose that the limitation of existing methods comes from the lack of comparison among individual knowledge sources, which leads to 
To avoid the suboptimal usage of knowledge by a blind concatenation of all sources, our method compares their confidence through individual inferences.
Specifically, we compare the reliability of each answer from DR- and QR-QA, then select the final answer $A_{ours}$ as follows: 
\begin{equation}
A_{ours} = \begin{cases}
  \mathbf{\hat{a}}_k & \text{if~} \text{P}(\mathbf{\hat{a}}_{k}|\mathbf{q},\mathbf{k}) \geq \text{P}(\mathbf{\hat{a}}_{d}|\mathbf{q},\mathbf{d}) \\
  \mathbf{\hat{a}}_d & \text{if~} \text{P}(\mathbf{\hat{a}}_k|\mathbf{q},\mathbf{k}) < \text{P}(\mathbf{\hat{a}}_d|\mathbf{q},\mathbf{d})
  \end{cases}
  \label{comparing_conf}
\end{equation}
where $\mathbf{\hat{a}}_k$ and $\mathbf{\hat{a}}_d$ are the decoded answers over QA pairs $\mathbf{k}$ and documents $\mathbf{d}$, respectively.
%In this way, the comparative advantage of every knowledge source is considered for the final decision.

The key point of our method is to find the effective measurement of the answer confidence, which is essentially the calibration problem.
The confidence score $\text{P}(\mathbf{\hat{a}}|\cdot)$ should be able to discern the accurate answer, by comparing the reliability of each knowledge.
We propose the way to find such $\text{P}(\mathbf{\hat{a}}|\cdot)$ in the next paragraph, based on our analysis of the important factors on documents and QA-pairs.

%[This is especiallly challenging because LMs are poorly calibrated in open-domain qa, and with poor calibration the selected result may be worse than the individual results] [For this reason we need good calibration measure, and we will show how to get good calibration measure and how to train qa model to produce them] 

%Taking account of multiple knowledge sources is a non-trivial problem. Method (1) provides an intuitive way, which is putting them all together as a single input, but it comes with the limitation that the knowledges from different sources might interfere each other. For example, \citet{oguz2020unik} reports that adding more knowledge sources can undermine overall performance in certain settings.
% [Additionally it requires longer context size for the aggregated input, which can also deteriorate the performance]
%To avoid the issues that arise from mixing up the knowledge, a straightforward alternative is to use each type of knowledge separately. 
%Method (2) follows this line of idea. 
%In \citet{lewis2021paq}, they consider QA-pair retrieval model as $\mathcal{F}$, and Open-book QA model on document as $\mathcal{G}$, in Eq.~(\ref{eq2}).
% the answer is first predicted by QA-pair retrieval () if their confidence is above threshold $\delta$. Otherwise, it is predicted by Open-book model on documents.
% in case the cosine similarity between $q$ and $k_{1}$ is below the arbitrary threshold $\theta$. 
%This method provides a reasonable compromise when the knowledge sources are prioritized so that the primary source (\eg, QA-pair) is differentiated from the secondary source to back off (\eg, document).
% for a certain design objective (e.g. computational efficiency).
%However, this method does not take every possible use of knowledge sources into account. 
%If the confidence of $\mathcal{F}$ is higher than the manually determined $\delta$, this method will ignore $\mathcal{G}$, regardless of the quality of the answers that might be obtained from $\mathcal{G}$.
% the back-off method will always prefer the QA-pair over the documents, regardless of the quality of the answer that might be obtained from documents.


% In contrast, our method ~~

% where $k_{1:m}$ is top $m$ knowledges from alternative source, $k_{1}$ is top 1 knowledge, $sim(q,k_{1})$ is cosine similarity between $q$ and $k_{1}$, and $\mathcal{S}(k_{1})$ is a simple knowledge-matching function that parses the answer from $k_{1}$. 
% Additionally, $cnf(q,k_{1:m})$ denotes the confidence estimate from language model when $q$ and $k_{1:m}$ are given.


%In terms of utilizing the complementarity, our method has advantage over method (1) and (2). 
%We separately infer answers from QA-pairs and documents, calculate and compare the reliability of each answer, then select the more reliable one as the final answer, as follows: 
%\begin{equation}
%A_{ours} = \begin{cases}
%  \mathcal{F}(q, \mathbf{k}) & \text{if~} P_{\mathcal{F}}(a|q,\mathbf{k}) \geq P_{\mathcal{G}}(a|q,\mathbf{d}) \\
%  \mathcal{G}(q, \mathbf{d}) & \text{if~} P_{\mathcal{F}}(a|q,\mathbf{k}) < P_{\mathcal{G}}(a|q,\mathbf{d})
%  \end{cases}
%\end{equation}



% \subsection{Calibration and Ensemble}


% Prior work has shown that a strong baseline for indomain selective prediction is MaxProb, a method
% that abstains based on the probability assigned
% by the model to its highest probability prediction
% (Hendrycks and Gimpel, 2017; Lakshminarayanan
% et al., 2017).

Prior work \cite{hendrycks2016baseline} has proposed MaxProb -- a method that uses the maximum probability of a classifier as the confidence estimator for selective prediction.
For extractive QA, existing works \cite{zhang2021knowing,si2022revisiting} adopt MaxProb as a baseline, by using the sum of the maximum logits of the start and end of the answer span.
Meanwhile, we focus on calibrating generative language models, where its output is a token sequence.
To apply MaxProb for generative LMs, 
we select the maximum probability at each step by the argmax function in Eq. (\ref{eq3}), which can be viewed as greedy decoding.
The scores of decoded tokens are aggregate by product, as follows:
% calculates the probability of a continuation Y that corresponds to the answer:
% Existing work for calibration~\cite{zhang2021knowing,jiang2021can,kadavath2022language} 
% computes the confidence of predicted answer $\mathbf{a}$, for question $\mathbf{q}$ and context $\mathbf{c}$ (either document or QA-pairs), using \textbf{LM probability}:
\begin{equation}
    \text{P}_{LM}(\mathbf{\hat{a}}|\mathbf{q},\mathbf{c}) =  \prod_{t=1}^{|\mathbf{\hat{a}}|} \text{P}_{LM}(\hat{a_t}|\mathbf{\hat{a}}_{<t}, \mathbf{q}, \mathbf{c})  % ^{1/|\mathbf{a}|}
    \label{lm_prob}
\end{equation}
where $\text{P}_{LM}(*)$ is the token probabilities obtained from LM head.
Since LM tends to underestimate the likelihood of longer texts, length normalization is essential as in \cite{adiwardana2020towards}.
To normalize as sequence lengths,\footnote{We empirically found that length normalization slightly improves the performance of Selective QA.} we take the geometric mean of the multiplicative terms, \ie, $\{ \text{P}_{LM}(\mathbf{\hat{a}}|\mathbf{q},\mathbf{c}) \}^{1/|\mathbf{\hat{a}}|}$.
% The geometric mean is taken for length normalization.

%To normalize the scores by sequence length, we take the geometric mean of the token-level scores.

However, this LM likelihood obtained by MaxProb has an inevitable problem.
MLE loss in Eq. (\ref{lm_loss}) enforces to train LM solely towards maximizing the likelihoods of observed sequences. 
Because the observed sequences (or labeled answers) can have diverse surface forms, MLE training inevitably leads to miscalibration.
In QA tasks, the sequence likelihood of QA models is reported to be often miscalibrated, or overconfident \cite{jiang2021can,kumar2019calibration}.
% overconfident~\cite{jiang2021can,kumar2019calibration}.
% because LM probabilities are trained solely for increasing on the true target tokens as shown in Eq. (\ref{lm_loss}).
% especially over short outputs \cite{murray2018correcting} and frequent words \cite{ott2018scaling}.

In Figure \ref{calibation_overfitting}, we also observe a consistent tendency in our open-domain QA task, where each line indicates the average confidence score of three estimates on correct predictions (solid line) and incorrect predictions (dashed line).
As the training steps increase, the scores of LM likelihood (red lines) increases monotonically, and even the gap between correct and incorrect predictions decreases.
We denote this problem as \textbf{calibration overfitting}, and hypothesis two causes (C1 and C2).
% \begin{itemize}
\begin{itemize}[leftmargin=0.4cm]
\setlength\itemsep{2pt}
\item C1: LM's objective maximizes the probabilities on answers regardless if the retrieved context is answerable or not, such that it is overconfident on unanswerable contexts.
% LM is trained towards maximizing the probabilities of ground truth texts, 
% such that the scores only increase without other objectives lowering on contexts that cannot answer the question.
\item C2: LM likelihood of a decoded output alone does not represent their uncertainty, while candidates unselected by greedy decoding can be a meaningful indicator of uncertainty.
% LM probability is estimated on a decoded answer $\mathbf{\hat{a}}$, while unselected candidates from decoder are a meaningful indicator of uncertainty.
\end{itemize}
% Assuming that answer candidates are given for multiple-choice QA, 


To deal with the above issues, we propose a new calibration approach of learning two measures: \textbf{Answerability} and \textbf{Consistency}, which are robust to calibration overfitting, as shown in Figure \ref{calibation_overfitting}.
For \textbf{C1}, we learn
% \paragraph{(C1) Lowering confidence for unanswerable passages:}
an answerability score, deciding whether the passage can answer the given question, which has been studied in Machine Reading Comprehension tasks~\cite{rajpurkar2018know}.
% to retrieve a passage that can answer the question.
Our contribution is to train to predict answerability for the question/context pair $(\mathbf{q},\mathbf{c})$ 
for the purpose of detecting the low confidence when the given context $\mathbf{c}$ cannot answer question $\mathbf{q}$.
%Calibration is context-dependent, so that modeling retrieved knowledge is essential in our QA task.
%To measure knowledge uncertainty, we adopt Answerability -- the probability a model assigns to the proposition that a given context contains answer $a^*$.
Training signals can be straightforwardly collected by whether the ground-truth answer $\mathbf{a}^*$ belongs to $\mathbf{c}$.
\begin{equation}
y_{\text{ans}} = \begin{cases}
  1, & \text{if~} \mathbf{a}^* ~ \text{belongs to}~ \mathbf{c} \\
  0, & \text{otherwise~}
  \end{cases}
  \label{answerability}
\end{equation}


% \paragraph{(C2) Lowering confidence for uncertain samples:}
For \textbf{C2}, we focus on sampling uncertainty.
The same decoded answer $\mathbf{\hat{a}}$ may have a high uncertainty, if a discarded candidate from the decoder is also highly plausible.
In contrast, the same answer has low uncertainty, if discarded candidates from the decoder are not plausible.

%Greedy decoding may generate a correct answer, but sampling uncertainty can be high, if a discarded candidate in the generation, an incorrect answer, is also highly plausible.
%In contrast, such uncertainty would be low, if the plausibility of wrong answers are much lower.
%The level of uncertainty can be leveraged in calibration, by lowering confidence when the sampling uncertainty is high.

\begin{figure}[t]
	\centering
	\includegraphics[width=68mm]{figures/figure_observation.pdf}
	\caption{Average scores of three confidence estimates over training epochs. While the solid line is confidence on correct answers, the dashed line is confidence on incorrect answers. Red: LM likelihood, Aqua: Answerability, Purple: Consistency.}
	\label{calibation_overfitting}
\end{figure}

To estimate such sampling uncertainty, we apply sampling-based decoding (temperature=1) generating a set of samples of size $N$, and measure sampling consistency.
% Similarly, \citet{lin2022teaching} calculate the average accuracy on Math questions in the same type (\ie, sub-task) as a proxy of uncertainty.
More formally, our supervision signal for uncertainty can be collected as:
\begin{equation}
    y_{\text{con}} = \frac{\text{frequency}(\mathbf{\hat{a}} = \mathbf{a}^*)}{N}
\end{equation}
where $\mathbf{\hat{a}}$ and $\mathbf{a}^*$ are the sampled output and the ground-truth, respectively.
$N$ is the number of samples, and we set $N=30$ in our experiment.



% Inspired, we generate $N$ samples given a question (at temperature = 1) from a warm-up QA model, and calculate the fraction of the correct answers over $N$, \ie, how consistently the sampled outputs from the model match the correct answers.

% Also, they demonstrated that language models can learn such scores well, by producing a binary value \cite{kadavath2022language} or a verbalized number \cite{lin2022teaching}.
% Inspired, we adopt and such score for open-domain QA

To supervise the above scores, we can build individual regression estimators $\text{P}_f$ and $\text{P}_g$, so that,
at inference time, we can use a calibration ensemble to combine the three scores:
\begin{equation}
    \begin{aligned}
     \text{Confidence}(\mathbf{\hat{a}}) = ~ & \text{P}_{LM}(\mathbf{\hat{a}}|\mathbf{x}) +
     \text{P}_f(\text{answerable}|\mathbf{x}) \\  + ~ &\text{P}_g(\text{consistent}|\mathbf{x})
    \end{aligned}
\end{equation}
where $\mathbf{x}$ is a pair of the context -- ($\mathbf{q}$, $\mathbf{c}$) or ($\mathbf{q}$, $\mathbf{k}$).


However, this approach requires to design and train additional estimators.
% training for two loss functions, 
% for $f$ and $g$ to compute confidence from each predicted pair $(x,y_{ans})$ and $(x,y_{con})$, respectively.
Meanwhile, some works supervise LM to verbally express the estimate scores, continued with an output sequence, \eg, sensibleness and safety \cite{thoppilan2022lamda} and uncertainty as question types \cite{lin2022teaching}.
The advantages of using verbal estimator are (1) no need to build separate networks for scoring, and (2) capturing interdependency between prediction and its uncertainty.
Specifically, we express $y_{ans}$ as either \textit{True} or \textit{False}, and convert real value $y_{con}$ into discrete words -- by partitioning it into equally sized quantiles (\ie, \textit{High}, \textit{Medium}, and \textit{Low}), as the following prompt:
% \textbf{Answerability}, P(Answerable=True $|q,d$) – The probability a model assigns to the proposition that a given context contains an answer.
\begin{figure}[h]
	\centering
	\includegraphics[width=72mm]{figures/output_template.pdf}
	\label{figure2}
\end{figure}
% \vspace{-3mm}

% \newpage


% With prompting, our generative model may capture interdependency among answer and estimated scores, while training once as in Eq. (\ref{lm_loss}) is redefined as follows:
After training with the prompt, we calculate two likelihoods of $\text{P}_f$ and $\text{P}_g$ at the inference time, as follows: 
\begin{equation}
    \begin{gathered}
    \text{P}_f(\text{answerable}|\mathbf{x}) = \text{P}_{LM}(\text{True}| \mathbf{x}) \\
    \text{P}_g(\text{consistent}|\mathbf{x}) = 1 \cdot \text{P}_{LM}(\text{High}| \mathbf{x}, \hat{y}_{ans}) \\ + 0.5 \cdot \text{P}_{LM}(\text{Medium}| \mathbf{x}, \hat{y}_{ans}) \\
    % \mathbf{x}=(\mathbf{q},\mathbf{c}), ~~~~ \mathbf{y}=(\mathbf{a}, y_{ans}, y_{con}) \\
    % \mathcal{L}(\mathbf{x},\mathbf{y})
    % = \sum_{i}^{T} \text{log}~\text{P}_{LM}( y_i | \mathbf{x})
    \end{gathered}
\end{equation}
where $\mathbf{x}$ is the context with the above prompt.
The final confidences are used for comparing two candidates in Eq. (\ref{comparing_conf}), then it decides the final answer.


%Now that we have two more sources to estimate confidence, how do we aggregate these estimations into the final verdict? 
%A naive baseline would be building estimator per each new source, e.g., $P_{Ans}$ and $P_{Con}$, and train an aggregation function, e.g., average of the three probabilities. 
%Another wild idea is teaching language models to express confidence, by estimating then aggregating these factors. 
%Pros for this approach is that LM may capture interdependency of three estimations, and would not require additional training for optimal aggregation. Cons is that all this in black-box.

% In our experiment, we observe that the two measures can be an indicator of whether the answer is more accurate.

% predict whether the model can answer correctly,
%While our goal is to predict the above confidence scores, the next question is \textit{how can we train the confidence scores?}
%The label of Answerability is boolean (\ie, True/False), and that of Sampling Consistency is a continuous value with a range of [0,1].
%In order to learn the two values with answer generation, we adopt linguistic calibration. 
%The previous works generate responses along with linguistic score
%such quality score \cite{thoppilan2022lamda} and estimated accuracy \cite{lin2022teaching}.




% Since the order of the text outputs may affect QA performance, we select the best order on development set, that is, Answerability -- Answer -- Consistency.




% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=75mm]{figures/figure2.pdf}
% 	\label{figure2}
% \end{figure}

% To obtain the confidence measures at inference time, we train our model and format its output as follows. (...training method, step by step)






==> tables/calibration2.tex <==

% \begin{table}[t]
% \setlength{\tabcolsep}{3pt}
% \centering
% \begin{tabular}{l|cc|cc}
% \noalign{\hrule height 1pt}
% \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{2}{c|}{\textbf{NQ}} & \multicolumn{2}{c}{\textbf{TQA}} \\
% \multicolumn{1}{c|}{} & $ECE_{\downarrow}$  & $AUC_{\downarrow}$  & $ECE_{\downarrow}$ & $AUC_{\downarrow}$ \\
% \noalign{\hrule height 1pt}
% FiD-KD (LM prob) & 0.303 & 0.266 & 0.160 & 0.100 \\ 
% ~ \kyungjae{+Temp Scaling} & 0.xx & 0.xx & 0.xx & 0.xx\\ 
% \hline
% \textsc{Ours (DR-QA)} & & & &  \\ 
% ~ (1) LM probability & 0.305  & 0.290  & 0.182 & 0.091  \\ 
% ~ (2) Answerability & 0.154   & 0.307 & 0.185 & 0.116 \\ 
% ~ (3) Consistency & \textbf{0.134} & 0.244  & \texbf{0.154} & 0.099 \\ 
% ~ (1+2+3) Ours & 0.163  & \textbf{0.240} & 0.168 & \textbf{0.088} \\ 
% \hline
% \textsc{Ours (QR-QA)} & & & &  \\ 
% ~ (1) LM probability & 0.396 & 0.390  & 0.326 & 0.209  \\ 
% ~ (2) Answerability & \textbf{0.126}  & 0.293 & 0.174 & 0.188  \\ 
% ~ (3) Consistency & 0.153 & 0.298 & \textbf{0.074} & 0.174 \\ 
% ~ (1+2+3) Ours & 0.147 & \textbf{0.289} & 0.170 & \textbf{0.171}  \\ 
% \noalign{\hrule height 1pt}
% \end{tabular}
% \caption{Calibration Evaluation: ECE $\&$ AUC of our methods, compared to DR-QA baseline (FiD-KD). ${\downarrow}$ means the lower the metric, the better the calibration is.}
% \label{calibration2}
% \end{table}

==> tables/retrieval_combined.tex <==

\begin{table}[t]
\centering
\setlength{\tabcolsep}{6pt}
\scalebox{0.9}{
\begin{tabular}{c|cc|cc|cc}
\noalign{\hrule height 1pt} 
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Metric}}} & \multicolumn{2}{c|}{\textbf{Documents}} & \multicolumn{2}{c|}{\textbf{QA-Pairs}} & \multicolumn{2}{c}{\textbf{Doc} $\oplus$ \textbf{QAP}} \\
\multicolumn{1}{c|}{} & NQ & TQA  & NQ & TQA & NQ & TQA 
 \\
% \multicolumn{1}{c}{Metric}  & NQ   & TQA  & NQ   & TQA   \\ 
\noalign{\hrule height 1pt}

Top-1 & 50.9 & 56.9  & 41.7  &  41.3 & 64.7 &  \\
Top-5  & 75.1 & 80.2 & 53.5 &  51.2 & 80.6 &   \\ 
Top-10 & 80.8 & 84.8 & 58.5 & 55.7 & 84.9 & \\  
Top-30 & 86.8 & 88.6 & 64.5 & 61.4 & 89.8 &   \\  
Top-50 & 88.7 & 89.7 & 67.2 & 64.0 & 91.1 &  \\

% Top-1 & 50.91 & 56.86  & 41.83  &  41.81   \\
% Top-5  & 75.12 & 80.22 & 53.46 &  51.15    \\ 
% Top-10 & 80.80 & 84.77 & 58.45 & 55.71  \\  
% Top-30 & 86.81 & 88.59 & 64.49 & 61.43     \\  
% Top-50 & 88.67 & 89.66 & 67.15 & 63.98   \\
\noalign{\hrule height 1pt} 
\end{tabular}}
\caption{Retrieval accuracy on test sets in NQ and TQA.}
\label{retrieval}
\end{table}


